Semantic-level Decentralized Multi-Robot Decision-Making using Probabilistic Macro-Observations

Robust environment perception is essential for decision-making on robots operating in complex domains. Intelligent task execution requires principled treatment of uncertainty sources in a robot's observation model. This is important not only for low-level observations (e.g., accelerometer data), but also for high-level observations such as semantic object labels. This paper formalizes the concept of macro-observations in Decentralized Partially Observable Semi-Markov Decision Processes (Dec-POSMDPs), allowing scalable semantic-level multi-robot decision making. A hierarchical Bayesian approach is used to model noise statistics of low-level classifier outputs, while simultaneously allowing sharing of domain noise characteristics between classes. Classification accuracy of the proposed macro-observation scheme, called Hierarchical Bayesian Noise Inference (HBNI), is shown to exceed existing methods. The macro-observation scheme is then integrated into a Dec-POSMDP planner, with hardware experiments running onboard a team of dynamic quadrotors in a challenging domain where noise-agnostic filtering fails. To the best of our knowledge, this is the first demonstration of a real-time, convolutional neural net-based classification framework running fully onboard a team of quadrotors in a multi-robot decision-making domain.

==> TemplateFiles/inc.tex <==
\IEEEoverridecommandlockouts \overrideIEEEmargins 
%\pagestyle{plain}

\usepackage{TemplateFiles/fullpage}
\usepackage[ruled,vlined,linesnumbered]{TemplateFiles/algorithm2e}
\usepackage{mathrsfs}
\usepackage{graphicx}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{array}
\usepackage{flafter}
%\usepackage{cite}
\usepackage{subfigure}
\usepackage{verbatim}
%\usepackage{bbm}
\usepackage[usenames]{color}
\usepackage[svgnames]{xcolor}
\usepackage{psfrag}
\usepackage{umoline}
\usepackage{hyperref}
%\usepackage{appendix} %[2009/09/02 v1.2b extra appendix facilities]
\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}	% This is needed for \newtheorem and proof environment.
%\usepackage{natbib} % for citing the papers with auther-year format in parantheses.

\providecommand{\citet}[1]{\citeauthor{#1}\,[\citeyear{#1}]}
\providecommand{\citep}[1]{\cite{#1}}

\newtheorem{thm}{Theorem}
\newtheorem{Def}{Definition}
\newtheorem{Problem}{Problem}
\newtheorem{Lem}{Lemma}
\newtheorem{Cor}{Corollary}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{property}{Property}
\newtheorem{Remark}{Remark}
\newtheorem{exmp}{Example}[section]
%\newenvironment{proof}[1][Proof]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

\newcommand{\TypeOfDoc}{IJRR} % This either can be TR or Conf or IJRR
\newcommand{\FinalFlag}{No} % This either can be No or Accepted

\graphicspath{{./figs/}}

\allowdisplaybreaks[1]

%\newcommand{\kXX}[1]{\color{blue} XX #1 XX \color{black}}
%\newcommand{\AXX}[1]{\color{orange} XX #1 XX \color{black}}
\newcommand{\aXX}[1]{\color{purple} #1 \color{black}}
